Deep Domain Confusion: Maximizing for Domain Invariance

Recent reports suggest that a generic supervised deep CNN model trained on a large-scale dataset reduces, but does not remove, dataset bias on a standard benchmark. Fine-tuning deep models in a new domain can require a significant amount of data, which for many applications is simply not available. We propose a new CNN architecture which introduces an adaptation layer and an additional domain confusion loss, to learn a representation that is both semantically meaningful and domain invariant. We additionally show that a domain confusion metric can be used for model selection to determine the dimension of an adaptation layer and the best position for the layer in the CNN architecture. Our proposed adaptation method offers empirical performance which exceeds previously published results on a standard benchmark visual domain adaptation task.

==> adaptation-algs.tex <==

% SVM parameter
\newcommand{\svmT}{\bm{\theta}}
\newcommand{\svmB}{b}
\newcommand{\svmAug}{\tilde{\svmT}}
%\newcommand{\svmAugAll}{\svmAug_{\text{all}}}
\newcommand{\svmAugAll}{\bm{\Theta}}

\begin{figure}
\begin{center}
\includegraphics[width=.7\linewidth]{figs/model-adapt}
\end{center}
\caption{Our proposed adaptation model.}
\label{fig:model}
\end{figure}

% Describe adaptation algorithms
%Many methods have been proposed for visual domain adaptation. 
% \ks{similar edit as in intro, see if this make sense}

\et{The plan here is to seriously tone down the discussion of the adaptation algorithms in favor of pushing our method, which is selecting a layer to adapt with using A-distance, then applying various adaptation techniques on top of that. Unfortunately we haven't gotten around to actually writing out that explanation yet. Reviewers may want to skip this section for now.}

We propose a general framework for selectively adapting the parameters of a convolutional neural network (CNN) whose representation and classifier weights are trained on a large-scale source domain, such as ImageNet.
Our framework adds a final domain-adaptive classification ``layer'' that takes the activations of one of the existing network's layers as input features. Note that the network cannot be effectively fine-tuned without access to more labeled target data. This adapted layer is a linear classifier that combines source and target training data using an adaptation method. To demonstrate the generality of our framework, we select a representative set of popular linear classifier adaptation approaches that we empirically evaluate in Section~\ref{sec:eval}. We separate our discussion into the set of supervised and unsupervised adaptation settings.

Below we denote the features extracted over the source domain as $\bm{X}$ and the features extracted over the target domain as $\tilde{\bm{X}}$. Similarly, we denote the source domain image classifier as $\bm{\theta}$ and the target domain image classifier as $\bm{\tilde{\theta}}$.

\subsection{Unsupervised Adaptation}
Many unsupervised adaptation techniques seek to minimize the distance between subspaces that represent the source and target domains. We denote these subspaces as $U$ and $\tilde{U}$, respectively.

{\bf GFK~\cite{gong-cvpr12}}
The Geodesic Flow Kernel (GFK) method~\cite{gong-cvpr12} is an unsupervised domain adaptation approach which seeks embeddings for the source and target points that minimize domain shift.
Inputs to the method are $U$ and $\tilde{U}$, lower-dimensional embeddings of the source and target domains (e.g. from principal component analysis).
The method constructs the geodesic flow $\phi(t)$ along the manifold of subspaces such that $U = \phi(0)$ and $\tilde{U} = \phi(1)$.
Finally, a transformation $G$ is constructed by computing
$
G =
\int_0^1 \phi(t) \phi(t)^{\intercal} dt
$
using a closed-form solution, and classification is performed by training an SVM on the source data $\bm{X}$ and transformed target data $G\tilde{\bm{X}}$.
\\\\
{\bf SA~\cite{sa}}
The Subspace Alignment (SA) method~\cite{sa} also begins with low-dimensional embeddings of the source and target domains $U$ and $\tilde{U}$, respectively.
It seeks to minimize in $M$, a transformation matrix, the objective
$ \| UM - \tilde{U} \|^2_F$.
The analytical solution to this objective is $M^* = U^{\intercal} \tilde{U}$.
Given $M^*$, an SVM is trained on source data $\bm{X}$ and transformed target data $U M^* \tilde{U}^{\intercal} \tilde{\bm{X}}$.


\subsection{Supervised Adaptation}

{\bf Late Fusion}
Perhaps the simplest supervised adaptation method is to independently train a source and target classifier and combine the scores of the two to create a final scoring function. 
We call this approach Late Fusion. It has been explored by many for a simple adaptation approach.
Let us denote the score from the source classifier as $v_s$ and the score from the target classifier as $v_t$.  For our experiments we explore two methods of combining these scores, which are described below:
\begin{itemize}
\item {\bf Max}: Produce the scores of both the source and target classifier and simply choose the max of the two as the final score for each example. Therefore, $v_{\text{adapt}} = \max(v_s, v_t)$.
\item {\bf Linear Interpolation}: Set the score for a particular example to equal the convex combination of the source and target classifier scores,  $v_{\text{adapt}} = (1-\alpha)v_{s} + \alpha v_{t}$. This method requires setting a hyperparameter, $\alpha$, which determines the weights of the source and target classifiers.
\end{itemize}

Late Fusion has two major advantages: it is easy to implement, and the source classifier it uses may be precomputed to make adaptation very fast. In the case of the linear interpolation combination rule, however, this method can potentially suffer from having a sensitive hyperparameter. We show a hyperparameter analysis in Section~\ref{sec:eval}.

{\bf \daume~\cite{daume}}
This simple feature replication method was proposed for domain adaptation by~\cite{daume}.
The method augments feature vectors with a source component, a target component, and a shared component.
Each source data point $\bm{x}$ is augmented to $\bm{x}' = (\bm{x}; \bm{x}; \bm{0})$,
and each target data point $\tilde{\bm{x}}$ is augmented to $\tilde{\bm{x}}' = (\tilde{\bm{x}}; \bm{0}; \tilde{\bm{x}})$.
Finally, an SVM is trained on the augmented source and target data---a relatively expensive procedure given the potentially large size of the source domain and the tripled augmented feature dimensionality.

{\bf PMT~\cite{aytar-iccv11}} 
This classifier adaptation method, Projective Model Transfer (PMT), proposed by~\cite{aytar-iccv11}, is a variant of adaptive SVM. It takes as input a classifier $\svmT$ pre-trained on the source domain.
PMT-SVM learns a target domain classifier $\svmAug$ by adding an extra term to the usual SVM objective which regularizes the angle
$
\alpha(\svmAug, \svmT) =
\cos^{-1}\left(
  \frac{
    \svmT^{\intercal} \svmAug
  }{
    \| \svmT \| \| \svmAug \|
  }
\right)
$
between the target and source hyperplanes.
This results in the following loss function:
\begin{align}
\mathcal{L}_{PMT}(\svmAug)
&=
\frac{1}{2} \| \svmAug \|^2_2
+
\frac{\Gamma}{2} \| \svmAug \|^2_2 \sin^2 \alpha(\svmAug, \svmT)
+
\ell_{hinge}(\tilde{\bm{X}}, \tilde{\bm{Y}}; \svmAug)
\enspace,
\end{align}
where
$
\ell_{hinge}(\bm{X}, \bm{Y}; \svmT)
$
denotes the SVM hinge loss of a data matrix
$\bm{X}$,
label vector
$\bm{Y}$,
and classifier hyperplane $\svmT$,
and $\Gamma$ is a hyperparameter which, as it increases, enforces more transfer from the source classifier.

{\bf MMDT~\cite{hoffman-iclr13}}
% \newcommand{\mat}[1]{\begin{bmatrix} #1 \end{bmatrix}}
\newcommand{\mat}[1]{#1}
\newcommand\datransform{\mat{A}}
The Max-margin Domain Transforms (MMDT) method from~\cite{hoffman-iclr13} jointly optimizes an SVM-like objective over a feature transformation matrix $\datransform$ mapping target points to the source feature space and classifier parameters $\svmT$ in the source feature space.
In particular, MMDT minimizes the following loss function (assuming a binary classification task to simplify notation, and with
$\ell_{hinge}$
defined as in PMT):
\begin{align}
\mathcal{L}_{MMDT}(\svmT, \datransform)
&=
\frac{1}{2} \| \svmT \|^2_2
+
\frac{1}{2} \| \datransform - \mat{I} \|^2_F
+
C_s
\ell_{hinge}(\bm{X}, \bm{Y}; \svmT)
+
C_t
\ell_{hinge}(\datransform \tilde{\bm{X}}, \tilde{\bm{Y}}; \svmT)
\enspace,
\end{align}
where $C_s$ and $C_t$ are hyperparameters controlling the importance of correctly classifying the source and target points (respectively).





==> analysis.tex <==
Our adaptation experiments show that our layer selection strategy, in concert with traditional domain adaptation methods,
can significantly increase performance and mitigate the effects of domain shift.
% It is important not only to evaluate overall method performance, but to understand when each adaptation method can and should be applied.
Depending on the characteristics of the problem at hand, our results suggest different methods may be most suitable.

If no labels exist in the target domain, then there are unsupervised adaptation
algorithms that are easy to use and fast to compute at adaptation time, yet
still achieve increased performance over source-only methods.

In the case where we have a large source dataset and a limited number of labeled target examples, it may be preferable to compute source classifier parameters in advance, then examine only the source parameters and the target data at adaptation time.
This would correspond to using our late fusion approach DLF which is unaffected by the number of data points in the source domain at adaptation time, and can thus be applied quickly.

Finally, If there are no computational constraints and there are very few labels in
the target domain, the best-performing supervised adaptation method is to use our layer selection technique with a classifier trained using the ``frustratingly easy'' approach originally proposed by \daume~\cite{daume}.

We conclude with an experimental verification of our A-distance layer selection strategy.
For each choice of layer from the CNN, we computed the A-distance between Imagenet and the webcam Office domain, and compared it to the multiclass performance of DFE for that domain shift.
The results of this experiment can be seen in Figure~\ref{fig:a-dist-eval}.
At least for this particular domain shift, A-distance appears strongly inversely correlated with the multiclass accuracy of DFE, thereby validating our layer selection strategy.
Note that the method in ~\cite{hoffman-iclr14} requires the practitioner to select the bridge layer; averaging the performance across layers is thus equivalent to using~\cite{hoffman-iclr14}, and achieves an accuracy of 62.7\%. Our method clearly improves on this strategy, achieving an accuracy of 69.9\% using the final layer.


==> decaf.tex <==
% Decaf description
\label{sec:decaf}
For our task we consider adapting between a large source domain and a target domain with few or or no labeled examples. 
A typical approach to domain adaptation or transfer learning with deep architectures is to take the representation learned via back-propagation on a large dataset, and then transfer the representation to a smaller dataset by fine-tuning, i.e. backpropagation at a lower learning rate \cite{rcnn,zeiler-arxiv-2013}.
However, fine-tuning requires an ample amount of labeled target data and so should not be expected to work well when we consider the very sparse label condition, such as the \textit{one-shot learning} scenario we evaluate below, where we have just one labeled example per category in the target domain.

In fact, in our experiments under this setting, fine-tuning, with the standard approach, actually reduces performance.
Specifically, on the ImageNet$\rightarrow$Webcam task reported in Section~\ref{sec:eval}, using the final output layer as a predictor in the target domain received 77\% accuracy, while using the final output layer after fine tuning produced a degraded accuracy of 75\%. In our experiments, the only clear way to avoid overfitting and reducing overall performance was to set the learning rates so low the model essentially did not change. This is unsurprising, as fine tuning a large set of parameters normally requires many additional labeled examples to be effective.

A separate method that was recently proposed for deep adaptation is called Deep Learning for domain adaptation by Interpolating between Domains (DLID)~\cite{ref:dlid}. This method learns multiple unsupervised deep models directly on the source, target, and combined datasets and uses a representation which is the concatenation of the outputs of each model as its adaptation approach. 
While this was shown to be an interesting approach, it is limited by its use of only convolutional deep layers and its focus on unsupervised learning for the majority of its training.

In general, unsupervised deep convolutional models have been unable to achieve the performance of supervised deep CNNs. However, training a supervised deep model requires sufficient labeled data. Our insight is that the extensive labeled data available in the source domain can be exploited using a supervised model without requiring a significant amount of labeled target data.

%% this was moved to the next section
%Therefore, we propose learning a supervised deep CNN using a large amount of source data. Then, we considering fixing the network and training a new final adaptation layer that takes as input the activations from both the source and target data. By using this hybrid approach we utilize the strong representation available from the supervised deep model trained on a large source dataset while requiring only enough target labeled data to train a shallow model with far fewer parameters. 


%For extracting features from the deep source model, we follow the setup of Donahue et al.~\cite{deeplearning-arxiv-2013}, which extracts a visual feature \textit{DeCAF} from the ImageNet-trained architecture of~\cite{supervision}.

% Following the successful experiments of~\cite{deeplearning-arxiv-2013}, our experiments in Section~\ref{sec:eval} take features computed from the fully-connected layers of the network: DeCAF$_6$ and DeCAF$_7$.
% We then go beyond the ``mid-level'' layers to explore DeCAF$_8$, the 1000-dimensional layer whose activations are fed into a soft-max unit to compute the label probabilities, as a basis for adaptation.


%Convolutional neural networks (CNNs) are a layered representation for learning features from and predicting statistics of visual data.
%CNN architectures had early practical success in handwritten digit recognition via supervised back-propagation~\cite{lecun89}.
%Powerful GPUs and GPU implementations accompanied by large datasets have enabled high-capacity CNNs to emerge as the current state-of-the-art visual classification method, with~\cite{supervision} demonstrating that an eight-layer architecture with over 60 million parameters achieves a top-5 error of 18.2\% on the ILSVRC-2012~\cite{ilsvrc2012} validation set, sparking great interest in this particular network.
%The network is trained by fully supervised back-propagation (as in~\cite{lecun89}) from raw RGB image pixels (of a fixed size of 224 $\times$ 224) to the desired output labels.
%The first five layers of the network are convolutional; i.e., the activation of any particular neuron is determined entirely by the pixel values within a particular window of the input image, and the filter weights are shared across every input pixel neighborhood to which the filter is applied.
%Each of the final three layers, on the other hand, are fully-connected to each neuron from the previous layer, making features taken from these layers ``global'' in the sense that they (potentially) depend on the entire input image.

